A new bright z=6.82 quasar discovered with VISTA: VHS J0411-0907

We present the discovery of a new $z \sim 6.8$ quasar discovered with the near-IR VISTA Hemisphere Survey (VHS) which has been spectroscopically confirmed by the ESO New Technology Telescope (NTT) and the Magellan telescope. This quasar has been selected by spectral energy distribution (SED) classification using near infrared data from VISTA, optical data from Pan-STARRS, and mid-IR data from WISE. The SED classification algorithm is used to statistically rank two classes; foreground Galactic low-mass stars and high redshift quasars, prior to spectroscopic observation. Forced photometry on Pan-STARRS pixels for VHS J0411-0907 allows to improve the SED classification reduced-$\chi^2$ and photometric redshift. VHS J0411-0907 ($z=6.82$, $y_{AB} = 20.1$ mag, $J_{AB} = 20.0$ mag) has the brightest J-band continuum magnitude of the nine known quasars at $z > 6.7$ and is currently the highest redshift quasar detected in the Pan-STARRS survey. This quasar has one of the lowest black hole mass ($M_{\rm{BH}}= (6.13 \pm 0.51)\times 10^8\:\mathrm{M_{\odot}}$) and the highest Eddington ratio ($2.37\pm0.22$) of the known quasars at $z>6.5$. The high Eddington ratio indicates that some very high-$z$ quasars are undergoing super Eddington accretion. We also present coefficients of the best polynomials fits for colours vs spectral type on the Pan-STARRS, VISTA and WISE system for MLT dwarfs and present a forecast for the expected numbers of quasars at $z>6.5$.

==> BD_pcoeffs_vs_colours_ps1-2MASS.tex <==
\begin{table}
\begin{tabular}{ccccccccc}
coeffs & ri & iz & zy & yJ & JH & HK & KW1 & W1W2 \\
p6 & nan & -2.10630864531e-07 & -6.93598250309e-08 & nan & 5.51399039625e-08 & nan & 5.23050522313e-08 & nan \\
p5 & -6.73133647868e-06 & 8.4892612586e-06 & 2.99443776434e-06 & nan & -1.92981619064e-06 & 1.05832275656e-06 & -1.88893654625e-06 & nan \\
p4 & 0.000461660756824 & -8.34620449249e-06 & 1.65046982831e-05 & 2.50462598467e-05 & -2.54980608346e-05 & -5.90861303847e-05 & -2.18532844251e-05 & nan \\
p3 & -0.0106658674079 & -0.00312462787061 & -0.0022405301519 & -0.00135480650507 & 0.00125229806742 & 0.000914723635697 & 0.00128881390325 & 0.000316707427909 \\
p2 & 0.0831107359401 & 0.0374785778292 & 0.0304083682588 & 0.0216619803719 & -0.00716680884242 & -0.00358008197262 & -0.0108006173998 & -0.00828128170284 \\
p1 & 0.0221488326683 & -0.00781703665719 & -0.0497276313227 & -0.0371793766369 & -0.00476168864292 & 0.0249262428081 & 0.0416387279814 & 0.07529563715 \\
p0 & 0.695897471336 & 0.33161553923 & 0.200624631744 & 0.236691538359 & 0.17203168007 & -0.281309500065 & -0.762427937295 & -0.638730216261 \\
\end{tabular}
\end{table}

